Topic Augmented Generator for Abstractive Summarization

Steady progress has been made in abstractive summarization with attention-based sequence-to-sequence learning models. In this paper, we propose a new decoder where the output summary is generated by conditioning on both the input text and the latent topics of the document. The latent topics, identified by a topic model such as LDA, reveals more global semantic information that can be used to bias the decoder to generate words. In particular, they enable the decoder to have access to additional word co-occurrence statistics captured at document corpus level. We empirically validate the advantage of the proposed approach on both the CNN/Daily Mail and the WikiHow datasets. Concretely, we attain strongly improved ROUGE scores when compared to state-of-the-art models.

==> results-caption.tex <==
% !TEX root = emnlp2018.tex
\subsection{Task 2: Image and Caption Retrieval}
We now study the usefulness of the learned word embeddings for the tasks of image and caption retrieval. Our hypothesis is that multimodal word embeddings will perform better for downstream tasks involving multimodal information. 
%%
{\setlength\tabcolsep{3pt}
\def\arraystretch{1.2}
\begin{table}
\caption{Results for image (I) $\leftrightarrow$ sentence (S) retrieval.}
    \label{fig1_caption}
\scriptsize
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
 \multirow{2}{*}{Models}  &       \multicolumn{3}{c|}{ I $\rightarrow$ S} & \multicolumn{3}{c|}{S $\rightarrow$ I} \\
  \cline{2-7}
     &   K=1    &  K=5  &  K=10  & K=1   & K=5  & K=10      \\
       \hline
      \textsc{sgns}  & 23.1&49.0&61.6&16.6&41.0&53.8\\
       \textsc{v-sgns} &  21.9&51.7&64.2&16.2&42.0&54.8  \\
    \textsc{iv-sgns (linear)}   &  22.7&50.5&61.7&17.1&42.6& 55.4 \\ \hline
      \ourmethodnameOne   &24.2&52.5&65.4&17.5&43.8&56.2\\
      \ourmethodnameTwo  &\textbf{25.7}&\textbf{55.7}&\textbf{67.7}&\textbf{18.4}&\textbf{44.9}&\textbf{56.9}\\
  \hline
    \end{tabular}
\end{table}}
%%%
\paragraph{Experimental setup}
We use the Flickr30K dataset~\citep{young2014image} containing 31,000 images and 155,000 sentences (5 captions per image). The sentences describe the images. The task is to identify the best sentence describing an image or to identify the best image depicting a sentence.  We follow the data split setting provided by \citet{karpathy2015deep}, in which 1,000 images are used for validation and 1,000 for testing. The rest is used for training. 

The retrieval models compute the proximity between the image features and the sentence embeddings. For image features, we use the pre-computed features provided by \citet{faghri2017vse++}, which are extracted from the FC7 layer of VGG-19 \citep{simonyan2014very}. These 4,096-dimensional features are then linearly mapped to 1,024-dimensional features. For sentences, we use an one GRU-layer over the sequences of the word embeddings, resulting in 1,024-dimensional sentence embeddings.  

We use a triplet loss to train the retrieval model such that the inner product between the corresponding image feature and the sentence is greater than the inner products with incorrect sentences (or images)~\cite{kiros2014unifying}. The linear mapping and the GRU layer are then optimized to minimize the loss. We use the ADAM optimizer with the learning rate of 0.0002 and divide it by 10 every 15 epochs and we train the model for 30 epochs. Note that we do not \emph{fine-tune} either the original visual feature or the word embeddings.

\paragraph{Results} Table~\ref{fig1_caption} summarizes the results. The evaluation metrics are accuracies at top-K (K=1, 5, or 10) retrieved sentences or images. Our model consistently outperforms \textsc{sgns}  and other competing multimodal methods, which provides additional support for the benefits of our approach. 
















